GSM-Plus: A Comprehensive Benchmark for Evaluating the Robustness of LLMs as Mathematical Problem Solvers

Large language models (LLMs) have achieved impressive performance across various mathematical reasoning benchmarks. However, there are increasing debates regarding whether these models truly understand and apply mathematical knowledge or merely rely on shortcuts for mathematical reasoning. One essential and frequently occurring evidence is that when the math questions are slightly changed, LLMs can behave incorrectly. This motivates us to evaluate the robustness of LLMs' math reasoning capability by testing a wide range of question variations. We introduce the adversarial grade school math (GSM-Plus) dataset, an extension of GSM8K augmented with various mathematical perturbations. Our experiments on 25 LLMs and 4 prompting techniques show that while LLMs exhibit different levels of math reasoning abilities, their performances are far from robust. In particular, even for problems that have been solved in GSM8K, LLMs can make mistakes when new statements are added or the question targets are altered. We also explore whether more robust performance can be achieved by composing existing prompting methods, in which we try an iterative method that generates and verifies each intermediate thought based on its reasoning goal and calculation result.

==> tables/baseline_comparison.tex <==

\begin{table*}[t!]
    \vspace{-1em}
	\scriptsize
	\sffamily
	\def\arraystretch{1.15}
	\setlength{\tabcolsep}{1.5pt}
	\begin{tabular*}{\textwidth}{|m{0.187\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.10\textwidth}|>{\centering\arraybackslash}m{0.10\textwidth}|>
    {\centering\arraybackslash}m{0.09\textwidth}|>
    {\centering\arraybackslash}m{0.10\textwidth}|}
		\hhline{|-|-------|}
  		\centering\arraybackslash\textbf{ROCStories} \linebreak Story Generation & Logically coherence & Relatedness \linebreak to inputs &  Grammar & Engagement & Character development & Clarify & Appropriate length  \\
            \hhline{|-|-------|}
		\citet{wang2020narrative}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
   			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark \\
            \hhline{|-|-------|}
		\citet{guan2022lot} &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
   			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark \\
   		\hhline{|-|-------|}
		\texttt{\textsc{CoEval} (Our)}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			% \cellcolor{pale_yellow!35} $\bm{\sim}$ &
			\cellcolor{pale_green!35} human-added  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
   			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark \\
		\hhline{:=:=======:}
  		\centering\arraybackslash\textbf{Self-Instruct} \linebreak Instruction Following & Completeness & Relevance to instructions &  Factual correctness & Information & Clarity & Politeness & \\
            \hhline{|-|-------|}
            \citet{wang2022self} &
                \cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & \\
      	\hhline{|-|-------|}
		\citet{vicuna2023}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
   			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & \\
      	\hhline{|-|-------|}
		\texttt{\textsc{CoEval} (Our)}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark & \\
		\hhline{:=:=======:}
		\centering\arraybackslash\textbf{ELI5} \linebreak Long-form QA & Overall usefulness & Factual \linebreak accuracy & Logically coherence & Simple \linebreak language & Example \linebreak usage  & & \\ 
  		\hhline{|-|-------|}
		% \hhline{:=:======:}
		\citet{LiRKWBCW20} &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark  & % $\bm{\sim}$
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & & \\
		\hhline{|-|-------|}
		\texttt{\citet{webgpt}} &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & & \\
			% \cellcolor{pale_red!35} human-annotated \\
		\hhline{|-|-------|}
		\texttt{\textsc{CoEval} (Our)}  &
			\cellcolor{pale_green!35} human-revised  &
   			\cellcolor{pale_green!35} human-added  &
			% \cellcolor{pale_yellow!35} $\bm{\sim}$ &
			\cellcolor{pale_green!35} human-added  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark & & \\
		\hhline{|-|-------|}
	\end{tabular*}
\caption{}\label{tab:baseline_comparison}
	\vspace{-2ex}
\end{table*}




==> tables/comparison_pot_cot.tex <==



\begin{table*}[!t] %{r}[0cm]{0pt}
    \centering\small
    \hspace{-2.4mm}
    \footnotesize
    \setlength{\tabcolsep}{6.5pt}
    \renewcommand{\arraystretch}{1.15}
    % \begin{adjustbox}{raise=-40mm}
    \resizebox{2\columnwidth}{!}{
    \begin{NiceTabular}{l|ccccccccc}
    % \specialrule{0em}{0pt}{-1pt}
    \toprule
    \textbf{Model}  &\textbf{GSM8K (S)} & \textbf{Val. Mod.} & \textbf{Digit Exp.} & \textbf{IDF Conv.} & \textbf{Sem. Para.} & \textbf{Comp. Inc.}  &  \textbf{Interf. Inj.} & \textbf{Ques. Trans.} \\
    \midrule  %   & \textbf{Rem.}
    $\text{GPT-4}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont c+}}}$  &  96.07 &  
\cellcolor{DarkGreen!55}5.09 & \cellcolor{DarkGreen!35}1.01 & \cellcolor{DarkGreen!55}5.09 & \cellcolor{lightred}-1.03 & \cellcolor{DarkGreen!75}15.3 & \cellcolor{DarkGreen!45}4.07 & \cellcolor{DarkGreen!65}11.22  \\
    $\text{GPT-4}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont p+}}}$  &  90.00 &  
\cellcolor{DarkGreen!35}2.47 & \cellcolor{DarkGreen!25}1.38 & \cellcolor{DarkGreen!65}8.87 & \cellcolor{DarkGreen!45}3.87 & \cellcolor{DarkGreen!55}7.61 & \cellcolor{DarkGreen!75}10.11 & \cellcolor{DarkGreen!25}1.38  \\  
    \midrule
    $\text{LLaMA-2-70B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont c+}}}$ & 66.67 &  \cellcolor{DarkGreen!18}1.47 & \cellcolor{DarkGreen!35}7.36 & \cellcolor{DarkGreen!65}35.29 & \cellcolor{DarkGreen!25}4.41 & \cellcolor{DarkGreen!75}51.48 & \cellcolor{DarkGreen!45}25.0 & \cellcolor{DarkGreen!55}30.88 \\
    $\text{LLaMA-2-70B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont p+}}}$ & 62.75  & \cellcolor{DarkGreen!35}20.32 & \cellcolor{DarkGreen!25}20.32 & \cellcolor{DarkGreen!55}31.25 & \cellcolor{DarkGreen!18}4.7 & \cellcolor{DarkGreen!75}50.01 & \cellcolor{DarkGreen!45}25.0 & \cellcolor{DarkGreen!65}40.64  \\ 
    \midrule
    $\text{CodeLlama-34B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont c+}}}$ & 45.10 & \cellcolor{DarkGreen!35}19.58 & \cellcolor{DarkGreen!25}17.41 & \cellcolor{DarkGreen!55}26.1 & \cellcolor{DarkGreen!18}8.69 & \cellcolor{DarkGreen!75}71.73 & \cellcolor{DarkGreen!45}21.75 & \cellcolor{DarkGreen!65}30.44 \\
    $\text{CodeLlama-34B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont p+}}}$ & 50.00 & \cellcolor{DarkGreen!25}11.76 & \cellcolor{DarkGreen!35}13.72 & \cellcolor{DarkGreen!45}25.5 & \cellcolor{lightred}-5.88 & \cellcolor{DarkGreen!75}54.9 & \cellcolor{DarkGreen!55}37.26 & \cellcolor{DarkGreen!65}52.94  \\
    % \midrule
    % \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source models in mathematics (7B)}}} \\
    % WizardMath~\citep{luo2023wizardmath} & 7B	 \\
    % MetaMath-Mistral  &  84.31  &  \\
    % MetaMath & 78.43  &  \\
    % Abel  & 61.76  & \\
    % LLEMMA~\citep{azerbayev2023llemma}  &  7B &	51.5 & \\
    \midrule
    $\text{MAmmoTH-7B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont c+}}}$    &
    59.80 & \cellcolor{DarkGreen!25}9.83 & \cellcolor{DarkGreen!35}18.03 & \cellcolor{DarkGreen!55}37.71 & \cellcolor{DarkGreen!18}4.92 & \cellcolor{DarkGreen!75}57.37 & \cellcolor{DarkGreen!65}45.9 & \cellcolor{DarkGreen!45}32.78\\  % overall: 42.15
    $\text{MAmmoTH-7B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont p+}}}$ & 
    51.96 & \cellcolor{lightred}-1.89 & \cellcolor{lightred}-13.2 & \cellcolor{DarkGreen!55}32.08 & \cellcolor{lightred}-3.77 & \cellcolor{DarkGreen!65}39.63 & \cellcolor{DarkGreen!75}49.06 & \cellcolor{DarkGreen!45}32.08 \\  % overall: 42.02
    $\text{MAmmoTH-7B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont p+sc}}}$ &  \\
    $\text{MAmmoTH-7B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont c+sc}}}$ &  \\
     $\text{MAmmoTH-7B}^{\text{ \textbf{\fontsize{8pt}{12pt}\selectfont LoT+}}}$ &  \\
    \bottomrule
    \end{NiceTabular}
    }
    % \end{adjustbox}
    \caption{The extent of accuracy decay (\%) observed in Language Models (LLMs) with chain-of-thoughts (\textbf{C+}), program-of-thoughts (\textbf{P+}) and ... approaches across different types of question variations. 
    Values highlighted in \hlgreen{green} indicate lower performance compared to the initial GSM8K set, with darker shades of green indicating larger decay degrees. Conversely, values highlighted in \hlred{red} indicate higher performance compared to the initial GSM8K set.  \qt{multiple dimension figure}}\label{exp:pot_vs_cot}
    % \vspace{-12mm}
\end{table*}



==> tables/comparison_pot_cot_v1.tex <==
\begin{table}[!t] %{r}[0cm]{0pt}
    \centering
    \hspace{-2.4mm}
    \footnotesize
    % \setlength{\tabcolsep}{6.5pt}
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{l|c|c|c}
    \toprule
    \textbf{Rule} & \textbf{Corr@P\&C} & \textbf{Corr@P} &  \textbf{Corr@C} \\\midrule
    GSM8K &  45.10 & ~~5.88  & 33.33 \\ 
    \midrule
    GSM++ &  31.23 & 10.08 & 23.24 \\ 
    \midrule
    Val. Mod. &  41.18 & 11.76 & 24.51   \\
    Digit Exp. &  45.10 & ~~9.80 & 17.65 \\
    IDF Conv. &  29.41 & ~~5.88 & 32.35 \\
    Sem. Para. &  46.08 & ~~6.86 & 20.59 \\
    Comp. Inc. & 15.69 & 15.69 & 18.63 \\
    Interf. Inj. & 15.69 & 10.78 & 24.51  \\
    Ques. Trans. & 25.49 & ~~9.80 & 24.51 \\
    
    \bottomrule
    \end{tabular}
    % \end{adjustbox}
    \caption{The overlap and non-overlap proportions of correctly answered questions between program-aid LLM (MAmmoTH-7B) and reasoning-path-enhanced LLM (MetaMath-7B).}ß
    \label{exp:potcot}
    % \vspace{-12mm}
\end{table}

% $^\ddag$



==> tables/finegrained_rewritting.tex <==



\begin{table*}[!t] %{r}[0cm]{0pt}
    \centering\small
    \hspace{-2.4mm}
    \footnotesize
    \setlength{\tabcolsep}{6.5pt}
    \renewcommand{\arraystretch}{1.15}
    % \begin{adjustbox}{raise=-40mm}
    \resizebox{2\columnwidth}{!}{
    \begin{NiceTabular}{l|cccc|ccc|c}  % tabular
    % \specialrule{0em}{0pt}{-1pt}
    \toprule
    & & \multicolumn{3}{c}{ \textbf{Numerical Variables}} & \multicolumn{3}{c}{\textbf{Known Conditions}} & \multicolumn{1}{c}{\textbf{Unknown Answer}} \\
    \hline
    \textbf{Model}  & \textbf{GSM8K (S)} & \textbf{Val. Mod.} & \textbf{Digit Exp.} & \textbf{IDF Conv.} & \textbf{Sem. Para.} & \textbf{Comp. Inc.}  &  \textbf{Interf. Inj.} & \textbf{Ques. Trans.} \\\midrule  %   & \textbf{Rem.}
    Human &    \\
    \midrule
   \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{closed-source models}}}  \\
GPT-4  & 96.07 & 
\cellcolor{DarkGreen!55}$\text{91.18}_{\text{5.1}}$ & \cellcolor{DarkGreen!35}$\text{95.1}_{\text{1.0}}$ & \cellcolor{DarkGreen!55}$\text{91.18}_{\text{5.1}}$ & \cellcolor{lightred}$\text{97.06}_{\text{-1.0}}$ & \cellcolor{DarkGreen!75}$\text{81.37}_{\text{15.3}}$ & \cellcolor{DarkGreen!45}$\text{92.16}_{\text{4.1}}$ & \cellcolor{DarkGreen!65}$\text{85.29}_{\text{11.2}}$   \\
GPT-3.5-Turbo & 77.45 &  
\cellcolor{DarkGreen!25}$\text{69.61}_{\text{10.1}}$ & \cellcolor{DarkGreen!35}$\text{68.63}_{\text{11.4}}$ & \cellcolor{DarkGreen!45}$\text{67.65}_{\text{12.7}}$ & \cellcolor{DarkGreen!18}$\text{74.51}_{\text{3.8}}$ & \cellcolor{DarkGreen!85}$\text{50.0}_{\text{35.4}}$ & \cellcolor{DarkGreen!70}$\text{61.76}_{\text{20.3}}$ & \cellcolor{DarkGreen!60}$\text{64.71}_{\text{16.4}}$   \\
    \midrule
    \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source general models}}}  &  \\
Mistral-7B &  49.02 & 
\cellcolor{DarkGreen!35}$\text{44.12}_{\text{10.0}}$ & \cellcolor{DarkGreen!25}$\text{44.12}_{\text{10.0}}$ & \cellcolor{DarkGreen!45}$\text{36.27}_{\text{26.0}}$ & \cellcolor{DarkGreen!18}$\text{45.1}_{\text{8.0}}$ & \cellcolor{DarkGreen!85}$\text{18.63}_{\text{62.0}}$ & \cellcolor{DarkGreen!60}$\text{34.31}_{\text{30.0}}$ & \cellcolor{DarkGreen!70}$\text{31.37}_{\text{36.0}}$   \\
    LLaMA-2-7B & 16.67 &  
\cellcolor{lightred}$\text{16.67}_{\text{0.0}}$ & \cellcolor{DarkGreen!55}$\text{10.78}_{\text{35.3}}$ & \cellcolor{DarkGreen!45}$\text{11.76}_{\text{29.5}}$ & \cellcolor{lightred}$\text{16.67}_{\text{0.0}}$ & \cellcolor{DarkGreen!75}$\text{2.94}_{\text{82.4}}$ & \cellcolor{DarkGreen!65}$\text{7.84}_{\text{53.0}}$ & \cellcolor{DarkGreen!35}$\text{13.73}_{\text{17.6}}$  \\
    CodeLlama-7B & 36.27 &
\cellcolor{DarkGreen!18}$\text{32.35}_{\text{10.8}}$ & \cellcolor{DarkGreen!25}$\text{31.37}_{\text{13.5}}$ & \cellcolor{DarkGreen!45}$\text{24.51}_{\text{32.4}}$ & \cellcolor{DarkGreen!35}$\text{29.41}_{\text{18.9}}$ & \cellcolor{DarkGreen!75}$\text{7.84}_{\text{78.4}}$ & \cellcolor{DarkGreen!55}$\text{14.71}_{\text{59.4}}$ & \cellcolor{DarkGreen!65}$\text{13.73}_{\text{62.1}}$ \\
    LLaMA-2-13B & 29.41 &  
\cellcolor{lightred}$\text{41.18}_{\text{-40.0}}$ & \cellcolor{DarkGreen!35}$\text{28.43}_{\text{3.3}}$ & \cellcolor{DarkGreen!65}$\text{18.63}_{\text{36.7}}$ & \cellcolor{lightred}$\text{34.31}_{\text{-16.7}}$ & \cellcolor{DarkGreen!75}$\text{10.78}_{\text{63.3}}$ & \cellcolor{DarkGreen!45}$\text{23.53}_{\text{20.0}}$ & \cellcolor{DarkGreen!55}$\text{22.55}_{\text{23.3}}$  \\
    CodeLlama-13B & 40.20 & 
\cellcolor{DarkGreen!35}$\text{35.29}_{\text{12.2}}$ & \cellcolor{DarkGreen!25}$\text{36.27}_{\text{9.8}}$ & \cellcolor{DarkGreen!45}$\text{28.43}_{\text{29.3}}$ & \cellcolor{lightred}$\text{40.2}_{\text{0.0}}$ & \cellcolor{DarkGreen!75}$\text{13.73}_{\text{65.8}}$ & \cellcolor{DarkGreen!55}$\text{19.61}_{\text{51.2}}$ & \cellcolor{DarkGreen!65}$\text{15.69}_{\text{61.0}}$ \\  
CodeLlama-34B & 50.00 & 
\cellcolor{DarkGreen!25}$\text{44.12}_{\text{11.8}}$ & \cellcolor{DarkGreen!35}$\text{43.14}_{\text{13.7}}$ & \cellcolor{DarkGreen!45}$\text{37.25}_{\text{25.5}}$ & \cellcolor{lightred}$\text{52.94}_{\text{-5.9}}$ & \cellcolor{DarkGreen!75}$\text{22.55}_{\text{54.9}}$ & \cellcolor{DarkGreen!55}$\text{31.37}_{\text{37.3}}$ & \cellcolor{DarkGreen!65}$\text{23.53}_{\text{52.9}}$  \\
    LLaMA-2-70B & 66.67 &
\cellcolor{DarkGreen!18}$\text{65.69}_{\text{1.5}}$ & \cellcolor{DarkGreen!35}$\text{61.76}_{\text{7.4}}$ & \cellcolor{DarkGreen!65}$\text{43.14}_{\text{35.3}}$ & \cellcolor{DarkGreen!25}$\text{63.73}_{\text{4.4}}$ & \cellcolor{DarkGreen!75}$\text{32.35}_{\text{51.5}}$ & \cellcolor{DarkGreen!45}$\text{50.0}_{\text{25.0}}$ & \cellcolor{DarkGreen!55}$\text{46.08}_{\text{30.9}}$ \\
    % CodeLlama~\citep{roziere2023code} &  &  \\
    \midrule
    \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source models in mathematics (7B)}}} \\
    % WizardMath~\citep{luo2023wizardmath} & 7B	 \\
    MetaMath-Mistral  &  84.31  & 
\cellcolor{DarkGreen!35}$\text{78.43}_{\text{7.0}}$ & \cellcolor{DarkGreen!25}$\text{81.37}_{\text{3.5}}$ & \cellcolor{DarkGreen!55}$\text{64.71}_{\text{23.2}}$ & \cellcolor{lightred}$\text{85.29}_{\text{-1.2}}$ & \cellcolor{DarkGreen!75}$\text{43.14}_{\text{48.8}}$ & \cellcolor{DarkGreen!45}$\text{64.71}_{\text{23.2}}$ & \cellcolor{DarkGreen!65}$\text{62.75}_{\text{25.6}}$ \\
    MetaMath & 78.43  & 
\cellcolor{DarkGreen!25}$\text{65.69}_{\text{16.2}}$ & \cellcolor{DarkGreen!35}$\text{62.75}_{\text{20.0}}$ & \cellcolor{DarkGreen!45}$\text{61.76}_{\text{21.3}}$ & \cellcolor{DarkGreen!18}$\text{66.67}_{\text{15.0}}$ & \cellcolor{DarkGreen!75}$\text{34.31}_{\text{56.3}}$ & \cellcolor{DarkGreen!65}$\text{40.2}_{\text{48.7}}$ & \cellcolor{DarkGreen!55}$\text{50.0}_{\text{36.2}}$ \\
    Abel  & 61.76  & 
\cellcolor{lightred}$\text{63.73}_{\text{-3.2}}$ & \cellcolor{DarkGreen!35}$\text{53.92}_{\text{12.7}}$ & \cellcolor{DarkGreen!45}$\text{46.08}_{\text{25.4}}$ & \cellcolor{DarkGreen!25}$\text{59.8}_{\text{3.2}}$ & \cellcolor{DarkGreen!75}$\text{29.41}_{\text{52.4}}$ & \cellcolor{DarkGreen!65}$\text{40.2}_{\text{34.9}}$ & \cellcolor{DarkGreen!55}$\text{44.12}_{\text{28.6}}$ \\
    % LLEMMA~\citep{azerbayev2023llemma}  &  7B &	51.5 & \\
    % https://github.com/EleutherAI/math-lm
    % https://github.com/GAIR-NLP/abel
    MAmmoTH  & 51.96 & 
\cellcolor{lightred}$\text{52.94}_{\text{-1.9}}$ & \cellcolor{lightred}$\text{58.82}_{\text{-13.2}}$ & \cellcolor{DarkGreen!55}$\text{35.29}_{\text{32.1}}$ & \cellcolor{lightred}$\text{53.92}_{\text{-3.8}}$ & \cellcolor{DarkGreen!65}$\text{31.37}_{\text{39.6}}$ & \cellcolor{DarkGreen!75}$\text{26.47}_{\text{49.1}}$ & \cellcolor{DarkGreen!45}$\text{35.29}_{\text{32.1}}$ \\
    ToRA & 75.49 & 
\cellcolor{DarkGreen!18}$\text{73.53}_{\text{2.6}}$ & \cellcolor{DarkGreen!35}$\text{67.65}_{\text{10.4}}$ & \cellcolor{DarkGreen!45}$\text{63.73}_{\text{15.6}}$ & \cellcolor{DarkGreen!25}$\text{71.57}_{\text{5.2}}$ & \cellcolor{DarkGreen!65}$\text{43.14}_{\text{42.9}}$ & \cellcolor{DarkGreen!75}$\text{23.53}_{\text{68.8}}$ & \cellcolor{DarkGreen!55}$\text{50.98}_{\text{32.5}}$ \\
MAmmoTH-Coder  & 73.53 &  \cellcolor{DarkGreen!35}$\text{62.75}_{\text{14.7}}$ & \cellcolor{DarkGreen!18}$\text{69.61}_{\text{5.3}}$ & \cellcolor{DarkGreen!45}$\text{50.98}_{\text{30.7}}$ & \cellcolor{DarkGreen!25}$\text{64.71}_{\text{12.0}}$ & \cellcolor{DarkGreen!75}$\text{35.29}_{\text{52.0}}$ & \cellcolor{DarkGreen!65}$\text{39.22}_{\text{46.7}}$ & \cellcolor{DarkGreen!55}$\text{50.0}_{\text{32.0}}$ \\
    % https://github.com/TIGER-AI-Lab/MAmmoTH/tree/main
    % ToRA-Code & 46.85 (72.6) & - & - \\
    SEGO & 76.47 & 
\cellcolor{DarkGreen!18}$\text{72.55}_{\text{5.1}}$ & \cellcolor{DarkGreen!35}$\text{69.61}_{\text{9.0}}$ & \cellcolor{DarkGreen!45}$\text{61.76}_{\text{19.2}}$ & \cellcolor{DarkGreen!25}$\text{70.59}_{\text{7.7}}$ & \cellcolor{DarkGreen!75}$\text{42.16}_{\text{44.9}}$ & \cellcolor{DarkGreen!55}$\text{49.02}_{\text{35.9}}$ & \cellcolor{DarkGreen!65}$\text{49.02}_{\text{35.9}}$ \\
    \midrule
    
    \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source models in mathematics (13B)}}} \\
    % WizardMath~\citep{luo2023wizardmath} & 13B	 \\
    MetaMath & 77.45 & 
\cellcolor{DarkGreen!35}$\text{67.65}_{\text{12.7}}$ & \cellcolor{DarkGreen!25}$\text{71.57}_{\text{7.6}}$ & \cellcolor{DarkGreen!45}$\text{54.9}_{\text{29.1}}$ & \cellcolor{lightred}$\text{79.41}_{\text{-2.5}}$ & \cellcolor{DarkGreen!75}$\text{36.27}_{\text{53.2}}$ & \cellcolor{DarkGreen!65}$\text{50.98}_{\text{34.2}}$ & \cellcolor{DarkGreen!55}$\text{52.94}_{\text{31.6}}$ \\
    Abel  & 71.56  & 
\cellcolor{lightred}$\text{73.53}_{\text{-2.8}}$ & \cellcolor{DarkGreen!35}$\text{65.69}_{\text{8.2}}$ & \cellcolor{DarkGreen!45}$\text{53.92}_{\text{24.7}}$ & \cellcolor{lightred}$\text{73.53}_{\text{-2.8}}$ & \cellcolor{DarkGreen!75}$\text{35.29}_{\text{50.7}}$ & \cellcolor{DarkGreen!65}$\text{50.0}_{\text{30.1}}$ & \cellcolor{DarkGreen!55}$\text{50.98}_{\text{28.8}}$ \\
    ToRA & 79.41  & 
\cellcolor{DarkGreen!25}$\text{72.55}_{\text{8.6}}$ & \cellcolor{DarkGreen!35}$\text{69.61}_{\text{12.3}}$ & \cellcolor{DarkGreen!45}$\text{67.65}_{\text{14.8}}$ & \cellcolor{DarkGreen!18}$\text{75.49}_{\text{4.9}}$ & \cellcolor{DarkGreen!65}$\text{48.04}_{\text{39.5}}$ & \cellcolor{DarkGreen!75}$\text{39.22}_{\text{50.6}}$ & \cellcolor{DarkGreen!55}$\text{57.84}_{\text{27.2}}$   \\
    MAmmoTH  & 64.71 & 
\cellcolor{DarkGreen!25}$\text{63.73}_{\text{1.5}}$ & \cellcolor{DarkGreen!35}$\text{61.76}_{\text{4.6}}$ & \cellcolor{DarkGreen!45}$\text{51.96}_{\text{19.7}}$ & \cellcolor{lightred}$\text{69.61}_{\text{-7.6}}$ & \cellcolor{DarkGreen!75}$\text{35.29}_{\text{45.5}}$ & \cellcolor{DarkGreen!65}$\text{41.18}_{\text{36.4}}$ & \cellcolor{DarkGreen!55}$\text{49.02}_{\text{24.2}}$ \\
MAmmoTH-Coder  & 75.49  & \cellcolor{DarkGreen!18}$\text{71.57}_{\text{5.2}}$ & \cellcolor{DarkGreen!35}$\text{66.67}_{\text{11.7}}$ & \cellcolor{DarkGreen!55}$\text{58.82}_{\text{22.1}}$ & \cellcolor{DarkGreen!25}$\text{67.65}_{\text{10.4}}$ & \cellcolor{DarkGreen!75}$\text{35.29}_{\text{53.3}}$ & \cellcolor{DarkGreen!45}$\text{58.82}_{\text{22.1}}$ & \cellcolor{DarkGreen!65}$\text{52.94}_{\text{29.9}}$ \\
    % ToRA-Code & 52.92 (75.8) & - & - \\52.94 & 58.82 & 35.29 & 53.92 & 31.37 & 26.47 & 35.29 &
    SEGO & 76.47 & 
\cellcolor{DarkGreen!25}$\text{72.55}_{\text{5.1}}$ & \cellcolor{DarkGreen!35}$\text{67.65}_{\text{11.5}}$ & \cellcolor{DarkGreen!45}$\text{65.69}_{\text{14.1}}$ & \cellcolor{lightred}$\text{76.47}_{\text{0.0}}$ & \cellcolor{DarkGreen!65}$\text{50.98}_{\text{33.3}}$ & \cellcolor{DarkGreen!75}$\text{48.04}_{\text{37.2}}$ & \cellcolor{DarkGreen!55}$\text{58.82}_{\text{23.1}}$\\
    \midrule
    
    \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source models in mathematics (70B)}}} \\
    MetaMath &  90.20 &
\cellcolor{DarkGreen!35}$\text{78.43}_{\text{13.0}}$ & \cellcolor{DarkGreen!18}$\text{84.31}_{\text{6.5}}$ & \cellcolor{DarkGreen!65}$\text{65.69}_{\text{27.2}}$ & \cellcolor{DarkGreen!25}$\text{83.33}_{\text{7.6}}$ & \cellcolor{DarkGreen!75}$\text{53.92}_{\text{40.2}}$ & \cellcolor{DarkGreen!45}$\text{69.61}_{\text{22.8}}$ & \cellcolor{DarkGreen!55}$\text{69.61}_{\text{22.8}}$  \\
    Abel  & 85.29 & 
\cellcolor{DarkGreen!25}$\text{81.37}_{\text{4.6}}$ & \cellcolor{DarkGreen!35}$\text{76.47}_{\text{10.3}}$ & \cellcolor{DarkGreen!65}$\text{64.71}_{\text{24.1}}$ & \cellcolor{lightred}$\text{86.27}_{\text{-1.1}}$ & \cellcolor{DarkGreen!75}$\text{55.88}_{\text{34.5}}$ & \cellcolor{DarkGreen!45}$\text{71.57}_{\text{16.1}}$ & \cellcolor{DarkGreen!55}$\text{68.63}_{\text{19.5}}$ \\
    \bottomrule
    \end{NiceTabular}}
    % \end{adjustbox}
    \caption{Comparison of testing accuracy to existing LLMs across various types of question variations. For each LLM, \textbf{worse} performance under these question variations is associated with \hlred{\textbf{darker}} cell colors. The subscript digit accompanying each accuracy value represents the decay rate (\%) in performance compared to the initial test data of GSM8K. The value with the \hlred{red background} indicates a slight increase in performance for the corresponding question variation compared to the original GSM8K test set.}
    \label{exp:fine-grained-rewritting}
    % \vspace{-12mm}
\end{table*}

% \setlength{\columnsep}{14pt}
% \begin{table*}[!t] %{r}[0cm]{0pt}
%     \centering\small
%     \hspace{-2.4mm}
%     \footnotesize
%     \setlength{\tabcolsep}{6.5pt}
%     \renewcommand{\arraystretch}{1.15}
%     % \begin{adjustbox}{raise=-40mm}
%     \resizebox{2\columnwidth}{!}{
%     \begin{tabular}{l|cccccccc}
%     % \specialrule{0em}{0pt}{-1pt}
%     \toprule
%     \textbf{Model}  & \textbf{GSM8K} & \textbf{Val. Mod.} & \textbf{Digit Exp.} & \textbf{IDF Conv.} & \textbf{Sem. Para.} & \textbf{Comp. Inc.}  &  \textbf{Interf. Inj.} & \textbf{Ques. Trans.} \\\midrule  %   & \textbf{Rem.}
%    \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{closed-source models}}}  \\
%     GPT-4  & 92.80 &  
%     \cellcolor{DarkGreen!62}91.18 & \cellcolor{DarkGreen!35}95.10 & \cellcolor{DarkGreen!62}91.18 & \cellcolor{DarkGreen!18}97.06 & \cellcolor{DarkGreen!90}81.37 & \cellcolor{DarkGreen!45}92.16 & \cellcolor{DarkGreen!75}85.29 \\
%     GPT-3.5-Turbo & 71.80 & 
%     \cellcolor{DarkGreen!25}69.61 & \cellcolor{DarkGreen!35}68.63 & \cellcolor{DarkGreen!45}67.65 & \cellcolor{DarkGreen!18}74.51 & \cellcolor{DarkGreen!90}50.00 & \cellcolor{DarkGreen!75}61.76 & \cellcolor{DarkGreen!62}64.71 \\
%     \midrule
%     \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source general models}}}  &  \\
%     Mistral-7B &  40.33 & 
%     \cellcolor{DarkGreen!35}44.12 & \cellcolor{DarkGreen!35}44.12 & \cellcolor{DarkGreen!45}36.27 & \cellcolor{DarkGreen!25}45.10 & \cellcolor{DarkGreen!90}18.63 & \cellcolor{DarkGreen!62}34.31 & \cellcolor{DarkGreen!75}31.37 \\
%     LLaMA-2-7B & 13.42 &  
%     \cellcolor{DarkGreen!25}16.67 & \cellcolor{DarkGreen!62}10.78 & \cellcolor{DarkGreen!45}11.76 & \cellcolor{DarkGreen!25}16.67 & \cellcolor{DarkGreen!90}~~2.94 & \cellcolor{DarkGreen!75}~~7.84 & \cellcolor{DarkGreen!35}13.73 \\
%     LLaMA-2-13B & 25.47 &  
%     \cellcolor{DarkGreen!13}41.18 & \cellcolor{DarkGreen!35}28.43 & \cellcolor{DarkGreen!75}18.63 & \cellcolor{DarkGreen!18}34.31 & \cellcolor{DarkGreen!90}10.78 & \cellcolor{DarkGreen!45}23.53 & \cellcolor{DarkGreen!62}22.55 \\
%     LLaMA-2-70B & 56.63 & 
%     \cellcolor{DarkGreen!18}65.69 & \cellcolor{DarkGreen!35}61.76 & \cellcolor{DarkGreen!75}43.14 & \cellcolor{DarkGreen!25}63.73 & \cellcolor{DarkGreen!90}32.35 & \cellcolor{DarkGreen!45}50.00 & \cellcolor{DarkGreen!62}46.08 \\
%     % CodeLlama~\citep{roziere2023code} &  &  \\
%     \midrule
%     \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source models in mathematics (7B)}}} \\
%     % WizardMath~\citep{luo2023wizardmath} & 7B	 \\
%     MetaMath-Mistral  &  78.01  & \cellcolor{DarkGreen!45}78.43 & \cellcolor{DarkGreen!35}81.37 & \cellcolor{DarkGreen!62}64.71 & \cellcolor{DarkGreen!25}85.29 & \cellcolor{DarkGreen!90}43.14 & \cellcolor{DarkGreen!62}64.71 & \cellcolor{DarkGreen!75}62.75 \\
%     MetaMath & 66.79  & \cellcolor{DarkGreen!25}65.69 & \cellcolor{DarkGreen!35}62.75 & \cellcolor{DarkGreen!45}61.76 & \cellcolor{DarkGreen!18}66.67 & \cellcolor{DarkGreen!90}34.31 & \cellcolor{DarkGreen!75}40.20 & \cellcolor{DarkGreen!62}50.00  \\
%     Abel  & 59.43  & \cellcolor{DarkGreen!13}63.73 & \cellcolor{DarkGreen!35}53.92 & \cellcolor{DarkGreen!45}46.08 & \cellcolor{DarkGreen!25}59.80 & \cellcolor{DarkGreen!90}29.41 & \cellcolor{DarkGreen!75}40.20 & \cellcolor{DarkGreen!62}44.12 \\
%     % LLEMMA~\citep{azerbayev2023llemma}  &  7B &	51.5 & \\
%     % https://github.com/EleutherAI/math-lm
%     % https://github.com/GAIR-NLP/abel
%     ToRA & 67.48 & \cellcolor{DarkGreen!18}73.53 & \cellcolor{DarkGreen!35}67.65 & \cellcolor{DarkGreen!45}63.73 & \cellcolor{DarkGreen!25}71.57 & \cellcolor{DarkGreen!75}43.14 & \cellcolor{DarkGreen!90}23.53 & \cellcolor{DarkGreen!62}50.98  \\
%     MAmmoTH  & 52.84 &  \cellcolor{DarkGreen!45}52.94 & \cellcolor{DarkGreen!25}58.82 & \cellcolor{DarkGreen!62}35.29 & \cellcolor{DarkGreen!35}53.92 & \cellcolor{DarkGreen!75}31.37 & \cellcolor{DarkGreen!90}26.47 & \cellcolor{DarkGreen!62}35.29 \\
%     % MAmmoTH-Coder  & 31.92 / 23.81 (59.4) &  - & - \\
%     % https://github.com/TIGER-AI-Lab/MAmmoTH/tree/main
%     % ToRA-Code & 46.85 (72.6) & - & - \\
%     SEGO & 68.69 & \cellcolor{DarkGreen!35}50.98 & \cellcolor{DarkGreen!25}52.94 & \cellcolor{DarkGreen!62}36.27 & \cellcolor{DarkGreen!45}44.12 & \cellcolor{DarkGreen!90}26.47 & \cellcolor{DarkGreen!75}33.33 & \cellcolor{DarkGreen!75}33.33  \\
%     \midrule
    
%     \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source models in mathematics (13B)}}} \\
%     % WizardMath~\citep{luo2023wizardmath} & 13B	 \\
%     MetaMath & 70.96 & \cellcolor{DarkGreen!35}67.65 & \cellcolor{DarkGreen!25}71.57 & \cellcolor{DarkGreen!45}54.90 & \cellcolor{DarkGreen!18}79.41 & \cellcolor{DarkGreen!90}36.27 & \cellcolor{DarkGreen!75}50.98 & \cellcolor{DarkGreen!62}52.94 \\
%     Abel  & 66.64  & \cellcolor{DarkGreen!18}73.53 & \cellcolor{DarkGreen!35}65.69 & \cellcolor{DarkGreen!45}53.92 & \cellcolor{DarkGreen!18}73.53 & \cellcolor{DarkGreen!90}35.29 & \cellcolor{DarkGreen!75}50.00 & \cellcolor{DarkGreen!62}50.98 \\
%     MAmmoTH  & 62.40 & \cellcolor{DarkGreen!25}63.73 & \cellcolor{DarkGreen!35}61.76 & \cellcolor{DarkGreen!45}51.96 & \cellcolor{DarkGreen!18}69.61 & \cellcolor{DarkGreen!90}35.29 & \cellcolor{DarkGreen!75}41.18 & \cellcolor{DarkGreen!62}49.02 \\
%     % MAmmoTH-Coder  & 42.76 / 39.35 (64.7)  & - & - \\
%     ToRA & 71.80  & \cellcolor{DarkGreen!25}72.55 & \cellcolor{DarkGreen!35}69.61 & \cellcolor{DarkGreen!45}67.65 & \cellcolor{DarkGreen!18}75.49 & \cellcolor{DarkGreen!75}48.04 & \cellcolor{DarkGreen!90}39.22 & \cellcolor{DarkGreen!62}57.84 \\
%     % ToRA-Code & 52.92 (75.8) & - & - \\52.94 & 58.82 & 35.29 & 53.92 & 31.37 & 26.47 & 35.29 &
%     SEGO & 72.50 & \cellcolor{DarkGreen!35}50.98 & \cellcolor{DarkGreen!25}51.96 & \cellcolor{DarkGreen!75}38.24 & \cellcolor{DarkGreen!45}47.06 & \cellcolor{DarkGreen!90}32.35 & \cellcolor{DarkGreen!90}32.35 & \cellcolor{DarkGreen!62}43.14 \\
%     \midrule
    
%     \multicolumn{6}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textit{open-source models in mathematics (70B)}}} \\
%     MetaMath~\citep{yu2023metamath} &  83.78 & \cellcolor{DarkGreen!45}78.43 & \cellcolor{DarkGreen!25}84.31 & \cellcolor{DarkGreen!75}65.69 & \cellcolor{DarkGreen!35}83.33 & \cellcolor{DarkGreen!90}53.92 & \cellcolor{DarkGreen!62}69.61 & \cellcolor{DarkGreen!62}69.61  \\
%     Abel  & 83.78 & \cellcolor{DarkGreen!25}81.37 & \cellcolor{DarkGreen!35}76.47 & \cellcolor{DarkGreen!75}64.71 & \cellcolor{DarkGreen!13}86.27 & \cellcolor{DarkGreen!90}55.88 & \cellcolor{DarkGreen!45}71.57 & \cellcolor{DarkGreen!62}68.63   \\
%     \bottomrule
%     \end{tabular}
%     }
%     % \end{adjustbox}
%     \caption{ Comparison of testing accuracy to existing LLMs across various types of question variations. For each LLM, \textbf{worse} performance under these question variations is associated with \textbf{darker} cell colors.}\label{exp:fine-grained-rewritting}
%     % \vspace{-12mm}
% \end{table*}

% $^\ddag$

==> tables/overall_ranking_bak.tex <==
\begin{table*}[!t]
    \centering
    \hspace{-2.4mm}
    \footnotesize
    \setlength{\tabcolsep}{6.5pt}
    \renewcommand{\arraystretch}{1.15}
    \resizebox{2\columnwidth}{!}{
    \begin{NiceTabular}{l|cccccccc}
    \toprule
    \textbf{Model}  & \textbf{Base} & \textbf{Math-SFT} & \textbf{Output Format} & \textbf{GSM8K} & \textbf{\datasetname} & \textbf{$\Delta$ PDR (\%)} $\downarrow$  & \textbf{ASP (\%)} $\uparrow$ \\\midrule
    Human & - &  - & NL Rationale & 96.77 &  97.65 & \cellcolor{lightergray}~-0.91  &  92.11 \\
    \midrule
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{PurpleRed}{\textit{closed-source models}}}}  \\
    GPT-4   & - &  Unknown & NL Rationale &  \textbf{93.25} &  \textbf{88.16}  & \cellcolor{lightergray}\textbf{~~5.46}  & \textbf{90.21} \\
    GPT-3.5-Turbo  & - & Unknown & NL Rationale & 73.62   &  63.18 & \cellcolor{lightergray}{14.18} & 72.81 \\  
    \midrule
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{PurpleRed}{\textit{open-source general models (7-70B)}}}}   \\
    Mistral-7B$^\ddag$ & - & No & NL Rationale & 39.58 & 29.12 & \cellcolor{lightergray}26.43  & 52.26\\
    LLaMA-2-7B$^\ddag$  & - & No & NL Rationale & 13.42 & ~~9.28  & \cellcolor{lightergray}{30.85} & 33.82 \\ 
    CodeLlama-7B$^\ddag$ &  LLaMA-2 &  No & Program & 25.32 &  17.20 & \cellcolor{lightergray}{32.07} & 45.40 \\ 
    \hdottedline
    LLaMA-2-13B$^\ddag$   & - & No & NL Rationale & 25.40  & 18.89  & \cellcolor{lightergray}25.63 & 44.78 \\ 
    CodeLlama-13B$^\ddag$  & LLaMA-2 &  No & Program & 35.78 & 27.03 & \cellcolor{lightergray}{32.76} & 54.01 \\ 
    \hdottedline
    CodeLlama-34B$^\ddag$  &  LLaMA-2 &  No & Program & 45.64 & 34.08 & \cellcolor{lightergray}25.33 & 56.24  \\
    \hdottedline
    LLaMA-2-70B$^\ddag$  & - & No & NL Rationale & \textbf{56.71} & \textbf{45.72} & \cellcolor{lightergray}\textbf{19.38} & \textbf{65.08} \\  
    \midrule
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{PurpleRed}{\textit{open-source models in mathematics (7B)}}}} \\
    MetaMath-Mistral & Mistral & MetaMathQA-395K & NL Rationale & \textbf{78.01}  & \textbf{61.22} &  \cellcolor{lightergray}\textbf{21.52} & \textbf{70.76} \\  
    MetaMath   &  LLaMA-2 &  MetaMathQA-395K & NL Rationale &  66.79  & 48.95 &  \cellcolor{lightergray}{26.71}  & 62.79 \\
    Abel   & LLaMA-2 &   Unreleased & NL Rationale &  59.51 & 42.25 & \cellcolor{lightergray}29.00  & 56.89 \\  
    ToRA  & LLaMA-2 & TORA-CORPUS-16k & Program+NL Rationale & 67.48  & 49.83 & \cellcolor{lightergray}{26.16} & 64.75 \\
    MAmmoTH   &  LLaMA-2 & MathInstruct-260K & Program & 52.84 & 36.73 & \cellcolor{lightergray}30.49 & 55.44 \\ 
    MAmmoTH-Coder & CodeLLaMA & MathInstruct-260K & Program & 59.89  & 44.27 & \cellcolor{lightergray}26.08 & 61.10 \\
    SEGO  & CodeLLaMA & GSM8K+MATH+AQuA & Program & 68.69  & 51.10 & \cellcolor{lightergray}{25.61} & 67.62 \\ 
    \hdottedline
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{PurpleRed}{\textit{open-source models in mathematics (13B)}}}} \\
    MetaMath  &  LLaMA-2 & MetaMathQA-395K & NL Rationale & 70.96  &  53.70  & \cellcolor{lightergray}{24.32} & 65.90 \\ 
    Abel  & LLaMA-2 &   Unreleased & NL Rationale & 66.72  & 51.62 &  \cellcolor{lightergray}22.63 & 63.90 \\  
    ToRA  & LLaMA-2  & TORA-CORPUS-16k & Program+NL Rationale & 71.80 & 54.72 &  \cellcolor{lightergray}{23.79} & 68.24 \\ 
    MAmmoTH &  LLaMA-2 & MathInstruct-260K & Program & 62.40 & 46.65 &  \cellcolor{lightergray}25.24 & 62.37 \\
    MAmmoTH-Coder & CodeLLaMA & MathInstruct-260K & Program & 64.90  & 50.25 &  \cellcolor{lightergray}22.57 & 65.02 \\
    SEGO  & CodeLLaMA & GSM8K+MATH+AQuA & Program & \textbf{72.50} & \textbf{56.34} & \cellcolor{lightergray}\textbf{22.29} & \textbf{70.62} \\ 
    \hdottedline
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{PurpleRed}{\textit{open-source models in mathematics (70B)}}}} \\
    MetaMath  &  LLaMA-2  & MetaMathQA-395K & NL Rationale & 82.41  & 64.23 &  \cellcolor{lightergray}{22.07} & 72.23 \\  
    Abel &  LLaMA-2  &   Unreleased &  NL Rationale & \textbf{83.85}  & \textbf{68.08} & \cellcolor{lightergray}\textbf{18.81} & \textbf{75.04} \\  
    MAmmoTH  &  LLaMA-2 & MathInstruct-260K & Program & 75.89 & 61.04 & \cellcolor{lightergray}{19.57} & 72.23 \\
    \arrayrulecolor{black}\bottomrule
    \end{NiceTabular}}
    \caption{Accuracy of current LLMs on GSM8K and \datasetname. Models marked with $^\ddag$ indicate their performance under an 8-shot setting. Math-SFT means whether the model has been fine-tuned on any math reasoning datasets.}
    \label{exp:main-expt} 
    \vspace{-3mm}
\end{table*}





==> tables/performance_on_testmini.tex <==
\begin{table*}[!t]
    \centering
    \hspace{-2.4mm}
    \footnotesize
    \setlength{\tabcolsep}{6.5pt}
    \renewcommand{\arraystretch}{1.15}
    \resizebox{1.7\columnwidth}{!}{
    \begin{NiceTabular}{lc|ccc|ccc}
    \toprule
     &  & \multicolumn{3}{c}{\textbf{Full Test Set}} & \multicolumn{3}{c}{\textbf{Mini Test Set}} \\
    \textbf{Model} & \textbf{GSM8K} & \textbf{\datasetname} & \textbf{$\Delta$ PDR (\%)} $\downarrow$  & \textbf{ASP (\%)} $\uparrow$ & \textbf{\datasetname} & \textbf{$\Delta$ PDR (\%)} $\downarrow$  & \textbf{ASP (\%)} $\uparrow$ \\
    \midrule
    Human  & 96.77 &  98.75 & \cellcolor{lightergray}~~-2.05  &  92.11 &  97.65 & \cellcolor{lightergray}~~-0.91  &  92.11 \\
    \midrule
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{DarkGreen}{\textit{closed-source models}}}}  \\
    GPT-4   &  \textbf{93.25} & \textbf{85.58} & \cellcolor{lightergray}{~~\textbf{8.23}} & \textbf{81.54} &  \textbf{85.08}  & \cellcolor{lightergray}\textbf{~~5.46}  & \textbf{84.12} \\
    GPT-3.5-Turbo  & 73.62  &  61.19 & \cellcolor{lightergray}{16.88} & 51.36 &  60.83 & \cellcolor{lightergray}{14.18} & 53.60 \\     
    \midrule
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{DarkGreen}{\textit{open-source general models (7-70B)}}}}   \\
    Mistral-7B$^\ddag$ & 39.58 & 26.18 & \cellcolor{lightergray}33.86 & 18.66 & 26.18 & \cellcolor{lightergray}26.43  & 21.08 \\
    LLaMA-2-7B$^\ddag$  & 13.42 & ~~8.12  & \cellcolor{lightergray}{39.49} & 3.97 & ~~7.96  & \cellcolor{lightergray}{30.85} & ~~4.54 \\ 
    CodeLlama-7B$^\ddag$ & 25.32 &  15.05 & \cellcolor{lightergray}{40.56} & ~10.0 &  13.91 & \cellcolor{lightergray}{31.66} & 11.43 \\ 
    \hdottedline
    LLaMA-2-13B$^\ddag$  & 25.40  & 16.57 & \cellcolor{lightergray}34.76 & ~~9.96 & 17.09  & \cellcolor{lightergray}25.63 & 11.37 \\ 
    CodeLlama-13B$^\ddag$  & 35.94  & 21.67 & \cellcolor{lightergray}39.71 & 15.22 & 22.01 & \cellcolor{lightergray}{32.83} & 17.26 \\    
    \hdottedline
    CodeLlama-34B$^\ddag$  & 45.64  & 21.67 & \cellcolor{lightergray}52.52 & 15.78 & 24.14 & \cellcolor{lightergray}47.11 & 17.86 \\
    \hdottedline
    LLaMA-2-70B$^\ddag$  & \textbf{56.71} & \textbf{40.04} & \cellcolor{lightergray}{\textbf{29.40}} & \textbf{32.31} & \textbf{39.77} & \cellcolor{lightergray}\textbf{19.38} & \textbf{36.90} \\  
    \midrule
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{DarkGreen}{\textit{open-source models in mathematics (7B)}}}} \\
    MetaMath-Mistral  & \textbf{78.01} & \textbf{56.25} & \cellcolor{lightergray}{\textbf{27.69}} & \textbf{50.56}  & \textbf{56.62} &  \cellcolor{lightergray}\textbf{21.52} & {56.55} \\  
    MetaMath   &  66.79   & 44.35 & \cellcolor{lightergray}33.53 & 37.91 & 48.95 &  \cellcolor{lightergray}{26.71}  & \textbf{62.79} \\
    Abel   &  59.51 & 37.09 & \cellcolor{lightergray}37.67 & 29.64 & 42.25 & \cellcolor{lightergray}29.00  & 33.81 \\      
    ToRA  & 67.48   & 43.60 & \cellcolor{lightergray}35.39 & 37.89  & 49.83 & \cellcolor{lightergray}{26.16} & 43.14 \\
    MAmmoTH & 52.84 & 32.14 & \cellcolor{lightergray}39.17 & 25.63 & 36.73 & \cellcolor{lightergray}30.49 & 29.30 \\ 
    MAmmoTH-Coder & 59.89  & 38.73 & \cellcolor{lightergray}35.33 & 32.02 & 44.27 & \cellcolor{lightergray}26.08 & 36.60 \\
    SEGO  &  68.69 & 44.71 & \cellcolor{lightergray}34.91 & 40.68 & 51.10 & \cellcolor{lightergray}{25.61} & 46.50 \\ 
    \hdottedline
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{DarkGreen}{\textit{open-source models in mathematics (13B)}}}} \\
    MetaMath  & 70.81 & 48.58 & \cellcolor{lightergray}{\textbf{31.39}} & 41.06 &  53.70  & \cellcolor{lightergray}{24.32} & 46.77 \\ 
    Abel  & 66.72  & 45.39 & \cellcolor{lightergray}31.97 & 37.45  & 51.62 &  \cellcolor{lightergray}22.63 & 42.63 \\  
    ToRA  & 71.80 & 47.88 & \cellcolor{lightergray}33.31 & 42.43 & 54.72 &  \cellcolor{lightergray}{23.79} & 48.29 \\ 
    MAmmoTH & 62.40 & 40.82 & \cellcolor{lightergray}34.58 & 34.05 & 46.65 &  \cellcolor{lightergray}25.24 & 38.91 \\
    MAmmoTH-Coder & 64.90   & 43.97 & \cellcolor{lightergray}32.25 & 36.93  & 50.25 &  \cellcolor{lightergray}22.57 & 42.20 \\
    SEGO  & \textbf{72.50} & \textbf{49.30} & \cellcolor{lightergray}32.00 & \textbf{44.79} & \textbf{56.34} & \cellcolor{lightergray}\textbf{22.29} & \textbf{51.19} \\ 
    \hdottedline
    \multicolumn{8}{c}{{\fontsize{10pt}{13.2pt}\selectfont \textcolor{DarkGreen}{\textit{open-source models in mathematics (70B)}}}} \\
    MetaMath  & 82.41   & 59.37 & \cellcolor{lightergray}\textbf{27.69} & 52.30  & 64.23 &  \cellcolor{lightergray}{22.07} & 59.53 \\  
    Abel & \textbf{83.85}  & \textbf{59.94} & \cellcolor{lightergray}28.52 & \textbf{55.31} & \textbf{68.08} & \cellcolor{lightergray}\textbf{18.81} & \textbf{62.86} \\  
    MAmmoTH  & 75.89 & 53.41 & \cellcolor{lightergray}{29.62} & {47.96} & 61.04 & \cellcolor{lightergray}{19.57} & 54.81 \\
    \arrayrulecolor{black}\bottomrule
    \end{NiceTabular}}
    \caption{Accuracy of current LLMs on GSM8K and the \textsc{minitest} of \datasetname.}
    \label{exp:testmini_perf} 
\end{table*}

==> tables/statistics.tex <==

% \setlength{\columnsep}{14pt}
\begin{table}[!t] %{r}[0cm]{0pt}
    \centering
    \hspace{-2.4mm}
    \footnotesize
    % \setlength{\tabcolsep}{6.5pt}
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{l|c|c|c}
    \toprule
    \textbf{RW Rule} &  \\\midrule
    Val. Mod. &  93.14 &  92.63 & 71.43  \\
    Digit Exp. &  95.10  & 95.88  & 80.00\\
    IDF Conv. & 89.22 & 92.31  & 8182 \\
    Sem. Para. &  100.00 & 97.06 & - \\
    Comp. Inc. & 86.27 &  84.62 & 80.90 \\
    Interf. Inj. & 86.27 & 95.45 & 71.43 \\
    Ques. Trans. & 34.31 & 88.57 & 83.58 \\
    \bottomrule
    \end{tabular}
    % \end{adjustbox}
    \caption{The efficacy of GPT-4 as a generator of test sample variations and the accuracy of GPT-4's answers to questions generated by itself and humans under various rewriting rules.}
    \label{tab:dataset}
    % \vspace{-12mm}
\end{table}

% $^\ddag$


